Bringing a Personal Point of View: Evaluating Dynamic 3D Gaussian Splatting for Egocentric Scene Reconstruction

Egocentric video provides a unique view into human perception and interaction, with growing relevance for augmented reality, robotics, and assistive technologies. However, rapid camera motion and complex scene dynamics pose major challenges for 3D reconstruction from this perspective. While 3D Gaussian Splatting (3DGS) has become a state-of-the-art method for efficient, high-quality novel view synthesis, variants, that focus on reconstructing dynamic scenes from monocular video are rarely evaluated on egocentric video. It remains unclear whether existing models generalize to this setting or if egocentric-specific solutions are needed. In this work, we evaluate dynamic monocular 3DGS models on egocentric and exocentric video using paired ego-exo recordings from the EgoExo4D dataset. We find that reconstruction quality is consistently lower in egocentric views. Analysis reveals that the difference in reconstruction quality, measured in peak signal-to-noise ratio, stems from the reconstruction of static, not dynamic, content. Our findings underscore current limitations and motivate the development of egocentric-specific approaches, while also highlighting the value of separately evaluating static and dynamic regions of a video.

==> figures/before_bmvc/dataset.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/dataset.png}
    \caption{First frame of each scene viewed from the exo perspective (left) and ego perspective (right). Ego perspective is obtained from the first exo camera. Top 8 scenes were selected randomly, while the bottom 2 are the manually-selected EgoGaussian scenes. Frames are shown after the undistortion step. Figure best viewed zoomed in.}
    \label{fig:dataset}
\end{figure*}

==> figures/before_bmvc/renderings.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/renderings_minn_uniandes.png}
    \caption{Ground truths and renderings of the models on 2 random and 1 EgoGaussian scene. Top row denotes the ground truth and the dynamic mask overlaid in green. As we can see, the models consistently reconstruct the dynamic regions of the scene with worse visual fidelity than the static regions. Figure best viewed zoomed in.}
    \label{fig:renderings}
\end{figure*}

==> old_sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> old_sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> old_sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> old_sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Method}
\label{sec:method}




==> sec/before_bmvc/0_abstract.tex <==
\begin{abstract}
Egocentric video offers a unique window into how humans perceive and interact with their surroundings, making it increasingly valuable for applications in augmented reality, robotics, and assistive technologies. However, egocentric footage poses unique challenges, such as rapid camera motion and complex scene dynamics, which can hinder 3D reconstruction. While 3D Gaussian Splatting (3DGS) has recently emerged as a state-of-the-art method for efficient, high-quality novel view synthesis, existing dynamic monocular variants are typically evaluated only on non-egocentric video. It remains unclear how well they generalize to the egocentric setting, and hence it is unknown whether models focused on the egocentric perspective are required. In this work, we evaluate the performance of dynamic monocular 3DGS models on egocentric video using paired ego-exo recordings from the EgoExo4D dataset. We find that, under current evaluation protocols, reconstruction quality is worse in the egocentric view compared to the exocentric view. By separately analyzing static and dynamic regions of the scene, our results suggest that the performance drop, measured in terms of peak signal-to-noise ratio, is due to difficulties in reconstructing static background content. These findings highlight the limitations of current models in egocentric scenarios and underline the need for egocentric-specific approaches. Our results also demonstrate the value of separate evaluation on static and dynamic regions for more nuanced insight into model performance.
\end{abstract}

==> sec/before_bmvc/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Egocentric, or first-person, video captures the visual experience of a person wearing a head-mounted camera. This type of data provides a natural window into how humans perceive and interact with their surroundings, making it especially valuable for applications in augmented reality \cite{ar_egocentric}, assistive technology \cite{assistive_corobot}, and robotics \cite{robotic_hand_ego}. Unlike third-person recordings, egocentric video closely reflects the visual input an agent receives while acting in the world. By using egocentric data, we can improve an agent's ability to understand and navigate the world from a first-person perspective, leading to more intuitive and efficient interactions in real-world scenarios \cite{assistive_corobot}.

However, egocentric data also presents unique challenges. The camera is subject to rapid, often unpredictable motion driven by head or body movement \cite{epic_fields}. At the same time, the scenes themselves are highly dynamic, frequently involving complex hand-object interactions \cite{EgoGaussian}. These factors make egocentric recordings particularly difficult to process and analyze.

To address these issues, large-scale egocentric datasets such as EPIC-Kitchens \cite{epic_kitchens, epic_kitchens_55}, HOI4D \cite{hoi4d}, and Ego4D \cite{ego4d} have driven advances in tasks like action recognition \cite{lsta}, action prediction \cite{egocentric_action_prediction}, and hand-object segmentation \cite{egohos}. Yet, one important direction remains largely underexplored: 3D novel view synthesis in egocentric settings. Tackling this gap is key to enabling more comprehensive spatial understanding and unlocking immersive applications such as augmented and virtual reality \cite{ego_lifter}.

3D Gaussian Splatting (3DGS) \cite{3dgs} has recently emerged as a state-of-the-art approach for high-quality and efficient 3D novel view synthesis. The method has found use cases in fields such as robotics \cite{mani_gaussian}. However, 3DGS was originally designed for static scenes and relies on multi-view inputs. As such, extensions have been proposed to the 3DGS framework to allow the handling of dynamic scenes viewed from a single camera (monocular) \cite{def3dgs, 4dgs, rtgs, EgoGaussian, 4d_rotor, wasserstein_gaussians, gaufre}. These methods, however, are commonly only evaluated on scenes filmed from a third-person, exocentric perspective, rather than from the egocentric perspective \cite{monocular_evaluation, d_nerf, dycheck, nerfies, nerf_ds}. As a result, it remains unclear how well these models perform when applied to egocentric video, and whether new models, specialized on the egocentric perspective, are needed.

To our knowledge, EgoGaussian \cite{EgoGaussian} is the only existing dynamic monocular 3DGS model specifically targeting egocentric vision. While EgoGaussian has demonstrated improved performance over monocular baselines on egocentric data, the evaluation is limited to egocentric recordings alone. It remains unclear whether the observed improvements stem from the model design, the data itself, or from other factors such as the evaluation protocol.

In this work, we aim to address this research gap and answer the question of how well existing monocular dynamic 3D Gaussian Splatting models perform when applied to egocentric data. To this end, we compare the existing models on paired recordings of the same scene from the ego and exo perspectives from the EgoExo4D dataset \cite{ego_exo}. Additionally, motivated by the fact that dynamic regions may be crucial to reconstruct correctly in practical applications \cite{endo_4dgs}, we compare the performance of the models on the static and dynamic regions separately. Overall, our main contributions can be summarized as follows:

\begin{enumerate}
    \item We compare the performance of three existing dynamic 3DGS models on paired ego-exo scenes from the EgoExo4D dataset.
    \item We compare the performance of existing models on static and dynamic regions of the scene. 
    \item We compare EgoGaussian to baseline monocular methods that do not focus on egocentric videos. 
\end{enumerate}

Our code and data will be released in the future. 


==> sec/before_bmvc/2_related_work.tex <==
\section{Related work}
\label{sec:related}

\textbf{Egocentric vision.} Egocentric, or first-person vision, focuses on capturing visual data from the viewpoint of a wearable or head-mounted camera. This special type of vision has recently garnered attention due to its importance for applications such as augmented reality \cite{ar_egocentric} and robotics \cite{assistive_corobot, robotic_hand_ego}. Although egocentric video is considered difficult due to issues such as the complexity of human actions \cite{ego_lifter, vscos} and varied camera motion \cite{epic_fields}, egocentric datasets such as Epic-Kitchens \cite{epic_kitchens, epic_kitchens_55} have helped advancements in fields such as video understanding and human-object interaction \cite{visor, egocentric_action_prediction}. In this work, we compare egocentric recordings to other types of recordings to verify whether the challenges posed by egocentric vision impact the performance of monocular 3D Gaussian Splatting methods. 

%First person, egocentric, vision has been of interest for fields such as augmented reality (AR) \cite{hoi4d} and robotics \cite{ego_exo, hoi4d}. Datasets, such as Epic-Kitchens \cite{epic_kitchens, epic_kitchens_55}, HOI4D \cite{hoi4d}, and Ego4D \cite{ego4d} caused advances in tasks such as video understanding and hand-object segmentation. However, the field of 3D Gaussian splatting from egocentric videos remains largely unexplored. To our knowledge, EgoGaussian \cite{EgoGaussian} is currently the only model focused on reconstructing 3D scenes from dynamic, egocentric videos. In this work, we compare EgoGaussian with other existing monocular models in egocentric settings. 

\textbf{3D Gaussian splatting for dynamic scenes.} 3D Gaussian Splatting (3DGS) \cite{3dgs} has recently emerged as a promising method for novel view synthesis of static scenes, outperforming existing NeRF-based approaches \cite{nerf, mip_nerf} in both rendering quality and speed \cite{3dgs}. However, 3DGS assumes the scene to be static, leading to artefacts, such as floaters, present in the reconstruction of dynamic scenes \cite{EgoGaussian, ego_lifter}. As such, special methods have been proposed to handle scene motion \cite{dyn3dgs, wasserstein_gaussians, relay_gs}. Of these, monocular methods \cite{def3dgs, 4dgs, rtgs, 4d_rotor, gaufre, gaussian_flow, spline_gs}, which require only a single viewpoint, are especially interesting \cite{monocular_evaluation}. Such monocular methods vary from describing the motion with a global deformation field \cite{def3dgs, 4dgs, gaufre}, assigning the motion to each Gaussian separately \cite{spline_gs, gaussian_flow}, or having no explicit motion model at all \cite{rtgs, 4d_rotor}. In this work, we focus on evaluating monocular models in egocentric dynamic scenes. 

% 3D Gaussian splatting (3DGS) \cite{3dgs} assumes a static scene, leading to artefacts, such as floaters, present in the reconstruction of dynamic scenes \cite{EgoGaussian, ego_lifter}. As such, special methods have been proposed to handle scene motion \cite{dyn3dgs, wasserstein_gaussians, relay_gs}. Of these, monocular methods \cite{def3dgs, 4dgs, rtgs, 4d_rotor, gaufre, gaussian_flow, spline_gs}, which require only a single viewpoint, are especially interesting \cite{monocular_evaluation}. Although these methods have shown strong performance on exocentric, third-person data \cite{monocular_evaluation}, it is currently unknown how well they perform in egocentric, first-person settings. In this work, we aim to benchmark existing monocular 3DGS models on dynamic, egocentric views and compare their performance on the same scenes viewed from an exocentric angle. 

\input{figures/dataset}

\textbf{Evaluation of existing models.} Various datasets are used for the evaluation of models for 3D Gaussian splatting from monocular videos with dynamics \cite{monocular_evaluation, d_nerf, nerfies, hyper_nerf, nerf_ds, dycheck}. D-Nerf \cite{d_nerf} contains synthetic scenes captured with a rapidly moving camera without motion blur. Nerfies \cite{nerfies}, HyperNerf \cite{hyper_nerf}, and DyCheck \cite{dycheck} all contain real-world recordings with a single camera of kitchen activities, animals, and other moving objects. Importantly, however, even the scenes involving human actors are not recorded from an egocentric perspective, but rather from an exocentric, third-person perspective. As such, it is currently unknown how well existing monocular 3DGS models perform when the recording is captured from an egocentric point of view and whether these models perform better or worse than with other types of recordings. In this work, we provide such an evaluation. 

\textbf{EgoGaussian.} To the best of our knowledge, EgoGaussian \cite{EgoGaussian} is currently the only publicly-available model that performs monocular 3DGS reconstruction of dynamic scenes focused on the egocentric perspective. Within a given clip, the model makes an explicit distinction between passive segments, where no object interaction happens, and active segments where the object is being manipulated by the actor\footnote{The EgoGaussian paper refers to these segments as \textit{static} and \textit{dynamic}. We change the notation to avoid confusion in the rest of this work.}. The passive segments are then used to initialize the static background and the object shape. The active segments are then used to refine the background and the object shape while also learning the pose of the moving object. The method also makes an additional assumption that the object motion is fully rigid, and the method does not attempt to model the actor. Overall, the model can only be applied to scenes where the active segments are in-between passive segments, only one object is being manipulated, and the object motion is rigid. In this work, we compare the reconstruction quality achieved by EgoGaussian to other monocular models that are not specifically designed for egocentric settings. 

Concurrent to our work, DeGauss \cite{degauss} has emerged as an alternative model for dynamic 3DGS focused on the egocentric perspective. However, the model does not currently have an existing implementation and is hence excluded from evaluation.

\textbf{Static and dynamic modeling.} Modeling the dynamic objects of the scene correctly is crucial for practical applications \cite{endo_4dgs}. Although the majority of dynamic and monocular 3DGS methods model static and dynamic regions of the video together \cite{def3dgs, 4dgs, rtgs, wasserstein_gaussians, 4d_rotor}, methods exist where the static and dynamic are being modeled separately \cite{EgoGaussian, gaufre}. In \cite{monocular_evaluation} the authors show, however, that existing methods reconstruct the static and dynamic regions similarly. Since the evaluation in \cite{monocular_evaluation} focuses on non-egocentric data, we perform a similar analysis in egocentric settings. In this way, we aim to show whether future models could benefit from modeling the static and dynamic regions separately. 




==> sec/before_bmvc/3_method.tex <==
\section{Method}
\label{sec:method}




==> sec/before_bmvc/4_results.tex <==
\section{Experiments}
\label{sec:results}

\subsection{Ego vs.\ Exo}

\input{figures/renderings}
\input{tables/full_results}


In this experimental section, we aim to answer whether reconstruction from egocentric data is indeed different from other types of data. To this end, we compare the performance of existing models on egocentric data against the performance on exocentric, third-person data. We choose to compare against exocentric recordings as they form a natural opposite of egocentric recordings.

\textbf{Dataset.} Proposed by Grauman \etal, Ego-Exo4D \cite{ego_exo} contains 1,286 hours of paired egocentric and exocentric recordings of skilled human activities. We select this dataset over alternative ego-exo datasets \cite{charades_ego, assembly101, h2o, home_action_genome, cmu_mmac} as it contains varied scenes and provides ground truth camera extrinsics and intrinsics as well as a semi-dense 3D point cloud, which can be used to initialize the Gaussians. The ground truth camera parameters and a semi-dense point cloud are especially important as they allow us to disentangle the performance of baselines from any errors that could stem from structure-from-motion algorithms, such as COLMAP \cite{colmap, EgoGaussian}.

We select 8 random clips, each exactly 300 frames (10 seconds) long, which approximately corresponds to the length of existing dynamic clips for the task of monocular 3DGS of dynamic scenes \cite{EgoGaussian}. Additionally, to evaluate EgoGaussian \cite{EgoGaussian}, we manually select 2 additional clips that meet the requirements of the model. First frames from both exo and ego views of the selected scenes are presented in \Cref{fig:dataset}. As we can see, exo views tend to capture more multi-view information of the scene and the exo cameras are static. These differences may cause the performance on ego and exo views to be different.

\textbf{Models.} Apart from EgoGaussian, we select three other baseline methods for monocular 3D Gaussian splatting of dynamics scenes. Those baselines are: Deformable-3DGS \cite{def3dgs}, 4DGS \cite{4dgs}, and RTGS \cite{rtgs}. We select Deformable-3DGS and 4DGS due to their strong performance on dynamic scenes as shown by Liang \etal \cite{monocular_evaluation}. Since both Deformable-3DGS and 4DGS define the motion with a global field \cite{def3dgs, 4dgs, monocular_evaluation}, we include RTGS to increase model variety, as it does not rely on an explicit motion model \cite{rtgs, monocular_evaluation}.

\textbf{Data preprocessing.} Both the ego and exo cameras used in the Ego-Exo4D dataset are fish eye and hence incompatible with the default 3D Gaussian splatting framework \cite{ego_exo, 3dgs, fisheye_gs}. To alleviate this issue, we undistort the frames using known camera intrinsics following the official guidelines \cite{ego_exo_undistortion}. However, this undistortion process introduces artifacts, resulting in black regions along the top and bottom of the exo images \cite{ego_exo_undistortion}, as also shown in \Cref{fig:dataset}. To determine valid pixels, we undistort a binary mask using the same transformation as the images. The undistorted mask is later used in the 3D Gaussian Splatting pipeline to exclude invalid regions.

\textbf{Evaluation protocol.} We compare the performance of models on time-synchronized ego and exocentric recordings of the same scene. For egocentric recordings, the training set is composed of subsequent even-indexed frames, the validation set comprises of frames whose index $i \equiv 1 \Mod{4}$, and the test set where $i \equiv 3 \Mod{4}$. This procedure is hence similar to Zhang \etal \cite{EgoGaussian}, but with a validation set extension that allows for a per-scene hyperparameter optimization. 

The exocentric cameras are static, and hence a recording from a single camera can not be used to train a 3D Gaussian Splatting model due to the lack of multi-view information \cite{3dgs_from_single_image}. Instead, we create the recording by randomly selecting a viewpoint at each index $i$. This setup ensures the recording is still monocular while providing enough 3D information to train the models, and is similar to the setup in D-Nerf \cite{d_nerf}. The recording is then split into train, test, and validation in the same way as for the egocentric case. 

\textbf{Evaluation metrics.} Following \cite{monocular_evaluation}, we report masked peak signal-to-noise ratio (mPSNR), masked structural similarity index measure (mSSIM), and masked learned perceptual image patch similarity (mLPIPS). For the eight random scenes, the mask corresponds to the undistorted binary mask defined earlier. For the EgoGaussian scenes, the mask further excludes the hand and body regions, as these are not within the reconstruction scope of EgoGaussian \cite{EgoGaussian}.

All metrics are computed on the test set. Each model is re-trained three times per scene using the same hyperparameters but different random seeds, allowing us to report standard deviations.

\input{tables/dynamic_results}
\input{tables/static_results}

\textbf{Hyperparameters.} We perform a random search to select per-scene hyperparameters for Deformable-3DGS, 4DGS, and RTGS. For 4DGS and RTGS, the search space includes parameter values from existing configurations. As Deformable-3DGS lacks such configurations, we instead search over the width and depth of the deformation network, as well as the total number of optimization steps. The exact search parameters for all models are provided in \Cref{sec:hyper_search_space}.

The search runs for a fixed duration of 4 hours per scene and per model. Each configuration is evaluated on the validation set, and the one with the highest masked PSNR is selected. All searches are performed on an NVIDIA A40 GPU located on the Delft AI Cluster \cite{daic}. Finally, it should be noted that training EgoGaussian on each scene exceeded 4 hours, hence no hyperparameter search was conducted for that model.


\textbf{Results.} The results of this experiment are presented in \Cref{tab:full_results}, where the metrics are averaged over the random and EgoGaussian scenes separately. As we can observe, the models almost always perform better on the exocentric recordings with very low variance in results. The only exception is the mPSNR score measured for the RTGS model on the EgoGaussian scenes. However, other metrics in this setting are still better for exocentric recordings. This difference in reconstruction quality between ego and exo shows that the reconstruction from egocentric perspective is more difficult for existing models on average.

The gap in mPSNR performance between ego and exo appears larger in the random scenes than the EgoGaussian scenes. However, it should be noted that the EgoGaussian clips consist of passive segments where no object interaction happens. Additionally, the hands are excluded from egocentric metric calculation and the object movement is fully rigid. These differences may cause the scene dynamics to be easier to reconstruct from the egocentric perspective, which could explain the mPSNR difference between ego and exo being smaller than in random scenes. This observation suggests that EgoGaussian clips may not be fully representative of models' performance on egocentric video. 

Comparing EgoGaussian to other models, we observe that it obtains worse reconstruction quality across all metrics. This is a surprising result, as in the original paper, EgoGaussian was shown to outperform both Deformable-3DGS and 4DGS on egocentric data \cite{EgoGaussian}. 

Example renderings are presented in \Cref{fig:renderings}. As we can see from the first two, random sequences, the overall reconstruction from the ego perspective is visibly worse than the exo view. In the basketball sequence, the difference is most visible due to the poor reconstruction of the basketball and the hands of the actor. Although the qualitative results reinforce the conclusion that the reconstruction from the egocentric perspective is more difficult, it is yet unclear whether this difference comes from the reconstruction of dynamic or static objects. 

% Finally, we note that the standard deviations 

\subsection{Dynamic vs.\ static}

Accurate dynamic modeling is essential for practical applications involving dynamic 3DGS \cite{endo_4dgs}. Additionally, dynamic objects pose different challenges than static objects and some methods model them separately \cite{EgoGaussian, gaufre}. In this section, we thus aim to answer whether the current methods reconstruct static and dynamic regions with the same accuracy.

\textbf{Dynamic masks.} We use Segment Anything 2 \cite{sam2} to manually annotate each dynamic object in selected clips. The mask for a given object at a given frame $i$ is only considered dynamic if the object visibly moved between frames $i$ and $i - 1$. Example resulting dynamic masks have been overlaid in green in \Cref{fig:renderings}.

\textbf{Evaluation metrics.} Similarly to the previous section, we use mPSNR, mSSIM, and mLPIPS to evaluate the models. The dynamic mask corresponds to the combined masks of all dynamic objects at the given frame. The static mask contains only the background, \ie all objects that are not currently moving. The static and dynamic masks are combined with the undistortion masks obtained previously to ensure only valid pixels are evaluated. 

\textbf{Results.} The results for the dynamic masks are presented in \Cref{tab:dynamic_results} while the results for the static masks in \Cref{tab:static_results}. Firstly, as we can see, the model variance remains low on both dynamic and static parts of the scene. Secondly, from \Cref{tab:dynamic_results}, it is no longer clear whether the reconstruction of dynamics is easier from the ego or exocentric views. 

In random scenes, the dynamic mPSNR for Deformable-3DGS and 4DGS is higher for the egocentric view. The egocentric mPSNR for the RTGS model is also much closer to the exocentric perspective than in \Cref{tab:full_results}. At the same time, as shown in \Cref{tab:static_results}, the static reconstruction is again of higher quality in terms of mPSNR in exocentric views. Both mSSIM and mLPIPS are better in the exocentric view on static and dynamic regions. Hence, these results suggest that the difference in reconstruction quality between ego and exo in terms of mPSNR comes from the reconstruction of static regions, not dynamic. 

In the EgoGaussian scenes, we observe that the dynamic reconstruction is almost always better in the egocentric case. This reinforces the previous hypothesis that the dynamics in EgoGaussian videos are easier to reconstruct in the egocentric view. Additionally, this further shows that the EgoGaussian clips may not form a representative sample of real, egocentric videos. 


%While the model variance remains low, as we can see from \Cref{tab:dynamic_results}, the reconstruction of dynamic objects is no longer clearly better in the exocentric case. In random scenes, the mPSNR is higher for both Def3DGS and 4DGS in the ego case. In EgoGaussian scenes, egocentric reconstruction is easier on average with most models performing better on this type of data. On the other hand, the reconstruction of static objects (\Cref{tab:static_results}) is again easier for all models in the exocentric case. 

Furthermore, the difference in performance between static and dynamic reconstruction is clearly visible both from the tables as well as \Cref{fig:renderings}. Across both egocentric and exocentric recordings, the models perform better when reconstructing the static regions of the scene. This highlights a key limitation of current methods in handling motion and suggests that future work should focus on explicitly improving dynamic scene understanding. 

\input{tables/egogaussian_ek_no_sub_results}
\input{tables/egogaussian_hoi4d_no_sub_results}

As with the previous results, EgoGaussian again performs worse than other baselines. The performance is worse in both the static and dynamic regions. This is again unexpected considering the original results \cite{EgoGaussian}.

\subsection{EgoGaussian vs.\ others}
\label{sec:egogaussian_vs_others} 

The performance of EgoGaussian, as shown in Tables \ref{tab:full_results}, \ref{tab:dynamic_results}, and \ref{tab:static_results}, is surprising. In the original paper, EgoGaussian outperformed 4DGS and Deformable-3DGS both quantitatively and qualitatively \cite{EgoGaussian}. However, the results obtained in this work do not support that finding. To validate our approach and ensure that our data processing and model training were conducted correctly, we evaluate EgoGaussian alongside the baselines on the original EgoGaussian data from the Epic-Kitchens \cite{epic_kitchens, epic_kitchens_55} and HOI4D \cite{hoi4d} datasets.



\textbf{Evaluation protocol.} We maintain the evaluation protocol from EgoGaussian and hence only split the data into a train and a test set. It is unknown which hyperparameters were used for the baselines in the EgoGaussian paper \cite{EgoGaussian}, hence we use default configurations. Both for the baselines and EgoGaussian we do not measure the reconstruction quality of body parts. Hence, we measure masked PSNR, SSIM, and LPIPS, similarly to previous experiments. 

Furthermore, it should be noted that in the official EgoGaussian evaluation, the masked out areas are simply zeroed which will lead to incorrect metric values \cite{EgoGaussian}. For example, for the PSNR calculation the masked out regions are treated as zero-error rather than being ignored. Additionally, EgoGaussian does not normalize input images to the $[-1, 1]$ range, which is necessary for the LPIPS computation \cite{lpips}. As in the previous sections, we instead use masked PSNR, SSIM, and LPIPS from \cite{monocular_evaluation} and \cite{dycheck}, which avoids these problems. We report the EgoGaussian results with (ours$^\dagger$) and without (ours$^*$) these changes in metrics. 

\textbf{Results.} The results on the Epic-Kitchens data are presented in \Cref{tab:egogaussian_ek_no_sub_results.tex} while the results on the HOI4D dataset are in \Cref{tab:egogaussian_hoi4d_no_sub_results.tex}. As we can observe from both tables, our results for the EgoGaussian model without metric changes (ours$^*$) closely match the original paper. However, the baselines perform much better than originally reported. Indeed, when comparing with updated metric calculations (ours$^\dagger$), the baselines tend to outperform EgoGaussian itself. These results therefore reinforce the findings from the previous section and show that the sudden difference in performance does not come from the data or the lack of hyperparameter tuning for EgoGaussian.

To better understand the issue, we contacted the authors of EgoGaussian, who kindly agreed to privately share the code used for the evaluation of Deformable-3DGS. Upon reviewing the code, we noticed what appears to be a bug related to the handling of timestamps when loading the model. We reached out to the authors to clarify whether this was indeed a bug, but did not receive a response.

% Additionally, it should be noted that we observed a common problem with both the Epic-Kitchens and HOI4D data where the frames may be duplicated due to poor lighting \cite{epic_kitchens_55}. This leads the testing set to be very similar to the training set. In turn, this might lead overfitting models to be preferred in the evaluation. We discuss this problem in more detail in ... . \todo{TODO: add this as an appendix/supplementary material.}



==> sec/before_bmvc/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textbf{Egocentric difficulty.} Results from \Cref{tab:full_results} suggest that the reconstruction from egocentric perspective is in fact harder for existing models than the reconstruction from the corresponding third-person views. However, perhaps surprisingly, based on the results from \Cref{tab:dynamic_results} and \Cref{tab:static_results}, the difficulty, measured in mPSNR, appears to come from the static regions of the scene. The dynamic regions are reconstructed with a similar mean mPSNR between ego and exocentric views, as shown in \Cref{tab:dynamic_results}.

\textbf{Dynamic difficulty.} Comparing the results from \Cref{tab:dynamic_results} and \Cref{tab:static_results} we observe that the reconstruction of dynamics is worse than the reconstruction of the static background. Existing methods, EgoGaussian included, reconstruct the static background with a higher visual fidelity than the dynamic object(s). These results may appear surprising as the study by Liang \etal \cite{monocular_evaluation} found that the performance of dynamic Gaussian methods `does not change much` after masking out the static components. Our results thus show that it is still worthwhile to evaluate static and dynamic regions separately when developing future models. Likewise, it might be beneficial to develop models where static and dynamic regions are modeled separately, such as in \cite{EgoGaussian, gaufre}.

\textbf{Limitations.} One might question the fairness of comparing egocentric and exocentric recordings due to inherent differences in aspects such as camera motion and multi-view coverage. Egocentric video is recorded from a moving, first-person perspective, while exocentric footage relies on multiple static cameras positioned around the scene. However, these differences are not artifacts of the evaluation setup but fundamental properties of each modality. Fixed-camera, multi-view exocentric recordings are standard in ego-exo datasets \cite{ego_exo, assembly101, h2o, home_action_genome, cmu_mmac}, and reflect how such data is typically collected in practice. Therefore, while the two modalities differ substantially, comparing them still offers meaningful insights into model performance under realistic and representative conditions.

Another limitation is reporting metrics in terms of mean value over all scenes. Since the performance may vary greatly between scenes due to their difficulty, outliers may skew the means. In \Cref{sec:per_scene_results}, we address this problem by comparing ego and exo performance per-scene and showing that the same conclusions hold.

Finally, we note that the ego-exo analysis included only two EgoGaussian scenes. This limitation stems primarily from time constraints and the lengthy training time required for EgoGaussian. Moreover, as our findings also suggest, these scenes include several constraints that make them less representative of real-world scenarios compared to the randomly selected scenes.

\textbf{Future work.} We showed that the reconstruction from an egocentric perspective is more difficult than the exocentric perspective for existing models. As such, these results highlight the need for models focused on egocentric vision for the task of monocular 3D Gaussian Splatting of dynamic scenes. We also showed that much of the disparity in mPSNR stems from the reconstruction of static regions. As such, future models focused on egocentric vision could address this gap in static reconstruction quality.

Additionally, the results included in this paper could be useful for the development of monocular models without focusing on egocentric perspective. We showed, contrary to previous findings \cite{monocular_evaluation}, that existing models reconstruct dynamic regions worse than static regions. This challenges the assumption that dynamic content is handled well by default, and points to a potential blind spot in current evaluation protocols. Future models could benefit from explicitly targeting dynamic reconstruction quality, and we recommend that future benchmarks distinguish between static and dynamic reconstruction performance to provide a more nuanced understanding of model behavior.




==> sec/before_bmvc/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we answered the question of how well existing, monocular dynamic 3D Gaussian Splatting models perform in egocentric settings. To this end, we compared the performance of existing models on paired ego-exo views from the EgoExo4D dataset. We found that models tend to achieve better reconstruction quality of scenes captured from the exocentric perspective. Additionally, our results suggest that this difference, measured in masked peak signal-to-noise ratio, comes from the reconstruction of static parts of the scene, as the dynamic regions tend to be reconstructed with similar quality between ego and exo views. Overall, our results show the need for models specialized in egocentric reconstruction, as current models struggle with the challenges posed by egocentric video.

==> sec/original/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/original/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/original/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/original/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/before_bmvc/dynamic_results.tex <==
\begin{table*}[t!]
\begin{adjustwidth}{-2cm}{-2cm}
    \centering
    \begin{tabular}{cccccccc}
        \cmidrule[0.5pt]{1-8}
         &  & \multicolumn{3}{c}{\textbf{Random scenes}} & \multicolumn{3}{c}{\textbf{EgoGaussian scenes}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
        \textbf{Model} & \textbf{View} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-8}
        EgoGaussian & Ego & - & - & - & 21.65 $\pm$ 1.03 & 0.59 $\pm$ 0.050 & 0.41 $\pm$ 0.047 \\
        \cmidrule{1-8}
        \multirow{2}{*}{Def3DGS} & Ego & \cellcolor{moderategrey}25.47 $\pm$ 0.05 & 0.65 $\pm$ 0.003 & 0.38 $\pm$ 0.004 & \cellcolor{moderategrey}24.58 $\pm$ 0.28 & 0.63 $\pm$ 0.010 & \cellcolor{moderategrey}0.36 $\pm$ 0.010 \\
        & Exo & 24.21 $\pm$ 0.10 & \cellcolor{moderategrey}0.70 $\pm$ 0.004 & \cellcolor{moderategrey}0.27 $\pm$ 0.002 & 22.70 $\pm$ 0.22 & \cellcolor{moderategrey}0.66 $\pm$ 0.004 & 0.37 $\pm$ 0.006  \\
        \cmidrule{1-8}
        \multirow{2}{*}{4DGS} & Ego & \cellcolor{moderategrey}24.56 $\pm$ 0.14 & 0.62 $\pm$ 0.004 & 0.42 $\pm$ 0.004 & \cellcolor{moderategrey}25.41 $\pm$ 0.26 & \cellcolor{moderategrey}0.66 $\pm$ 0.006 & \cellcolor{moderategrey}0.35 $\pm$ 0.008 \\
        & Exo & 24.05 $\pm$ 0.13 & \cellcolor{moderategrey}0.71 $\pm$ 0.005 & \cellcolor{moderategrey}0.28 $\pm$ 0.004 & 22.72 $\pm$ 0.39 & 0.64 $\pm$ 0.011 & 0.40 $\pm$ 0.010 \\
        \cmidrule{1-8}
        \multirow{2}{*}{RTGS} & Ego & 25.33 $\pm$ 0.05 & 0.65 $\pm$ 0.001 & 0.38 $\pm$ 0.002 & \cellcolor{moderategrey}26.29 $\pm$ 0.15 & \cellcolor{moderategrey}0.67 $\pm$ 0.010 & \cellcolor{moderategrey}0.32 $\pm$ 0.006 \\
        & Exo & \cellcolor{moderategrey}25.60 $\pm$ 0.43 & \cellcolor{moderategrey}0.75 $\pm$ 0.009 & \cellcolor{moderategrey}0.21 $\pm$ 0.008 & 23.42 $\pm$ 0.12 & 0.66 $\pm$ 0.003 & 0.34 $\pm$ 0.010 \\
        \cmidrule[0.5pt]{1-8}
    \end{tabular}
\end{adjustwidth}
    \caption{The performance of selected models on dynamic masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Average performance over 3 training runs is reported alongside the standard deviation. Numbers in grey represent whether the performance was better on the ego or exo view. As we can see, the models perform similarly on ego and exo views and there is no clear answer whether ego or exo is easier.}
    \label{tab:dynamic_results}
\end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian \cite{EgoGaussian} & Ego & - & - & - & 20.64 & 0.54 & 0.46 \\
%         \hline
%         \multirow{2}{*}{Def3DGS \cite{def3dgs}} & Ego & \textbf{25.49} & 0.65 & 0.33 & \textbf{25.25} & 0.65 & \textbf{0.30} \\
%         & Exo & 24.34 & \textbf{0.70} & \textbf{0.28} & 22.95 & \textbf{0.67} & 0.35  \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & \textbf{24.30} & 0.61 & 0.43 & \textbf{26.23} & \textbf{0.69} & \textbf{0.34} \\
%         & Exo & 23.00 & \textbf{0.67} & \textbf{0.31} & 20.07 & 0.57 & 0.44 \\
%         \hline
%         \multirow{2}{*}{RTGS \cite{rtgs}} & Ego & 25.65 & 0.66 & 0.36 & \textbf{26.50} & \textbf{0.67} & \textbf{0.30} \\
%         & Exo & \textbf{26.07} & \textbf{0.77} & \textbf{0.20} & 23.01 & 0.65 & 0.34 \\
%         \hline
%     \end{tabular}
%     \caption{The performance of selected models on dynamic masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Bolded numbers represent whether the performance was better on the ego or exo view. As we can see, the models perform similarly on ego and exo views and there is no clear answer as to whether ego or exo is easier.}
%     \label{tab:dynamic_results}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & \textbf{24.73} & 0.63 & 0.41 & \textbf{25.36} & \textbf{0.65} & \textbf{0.36} \\
%         & Exo & 24.27 & \textbf{0.72} & \textbf{0.28} & 22.52 & 0.64 & 0.40 \\
%         \hline
%     \end{tabular}
%     \caption{after hypersearch}
%     \label{tab:dynamic_after_hypersearch}
% \end{table*}



==> tables/before_bmvc/egogaussian_ek_no_sub_results.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{ccccccc}
        \cmidrule[0.5pt]{1-7}
         & \multicolumn{3}{c}{\textbf{Passive segments}} & \multicolumn{3}{c}{\textbf{Active segments}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        \textbf{Model} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-7}
        EgoGaussian (original) & 28.33 & 0.85 & 0.19 & 28.34 & 0.88 & 0.17 \\
        EgoGaussian (ours$^*$) & 28.76 & 0.86 & 0.18 & 30.55 & 0.89 & 0.15 \\
        EgoGaussian (ours$^\dagger$) & 28.61 & 0.85 & 0.25 & 30.35 & 0.88 & 0.22 \\
        \cmidrule{1-7}
        Deformable-3DGS (original) & 27.63 & 0.86 & 0.17 & 23.27 & 0.82 & 0.21 \\
        Deformable-3DGS (ours$^\dagger$) & \cellcolor{moderategrey}37.54 & \cellcolor{moderategrey}0.96 & \cellcolor{moderategrey}0.12 & \cellcolor{moderategrey}32.94 & \cellcolor{moderategrey}0.94 & \cellcolor{moderategrey}0.16 \\
        \cmidrule{1-7}
        4DGS (original) & 28.90 & 0.87 & 0.16 & 23.13 & 0.80 & 0.23 \\
        4DGS (ours$^\dagger$) & 34.40 & 0.93 & 0.18 & 29.61 & 0.89 & 0.23 \\
        \cmidrule[0.5pt]{1-7}
    \end{tabular}
    \caption{The performance of EgoGaussian and the other baselines on the original EgoGaussian Epic-Kitchens data \cite{epic_kitchens, EgoGaussian}. Ours$^*$ represents the results without metric changes and ours$^\dagger$ represents with the metric changes. Numbers denoted in grey represent the best scoring method across ours$^\dagger$ evaluations. As we can observe, ours$^*$ implementation of EgoGaussian scores similarly to the original. However, we observe that the baselines perform similarly or better than EgoGaussian, contrary to the original findings.}
    \label{tab:egogaussian_ek_no_sub_results.tex}
\end{table*}

==> tables/before_bmvc/egogaussian_hoi4d_no_sub_results.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{ccccccc}
        \cmidrule[0.5pt]{1-7}
         & \multicolumn{3}{c}{\textbf{Passive segments}} & \multicolumn{3}{c}{\textbf{Active segments}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        \textbf{Model} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-7}
        EgoGaussian (original) & 30.99 & 0.96 & 0.08 & 30.33 & 0.95 & 0.09 \\
        EgoGaussian (ours$^*$) & 30.52 & 0.96 & 0.09 & 31.12 & 0.96 & 0.09 \\
        EgoGaussian (ours$^\dagger$) & 30.43 & 0.95 & 0.13 & 30.97 & 0.95 & 0.13 \\
        \cmidrule{1-7}
        Deformable-3DGS (original) & 28.09 & 0.94 & 0.08 & 26.92 & 0.94 & 0.10 \\
        Deformable-3DGS (ours$^\dagger$) & 34.38 & \cellcolor{moderategrey}0.97 & \cellcolor{moderategrey}0.08 & 33.06 & 0.96 & \cellcolor{moderategrey}0.10 \\
        \cmidrule{1-7}
        4DGS (original)& 28.69 & 0.94 & 0.08 & 27.33 & 0.94 & 0.10 \\
        4DGS (ours$^\dagger$) & \cellcolor{moderategrey}36.73 & \cellcolor{moderategrey}0.97 & 0.09 & \cellcolor{moderategrey}35.13 & \cellcolor{moderategrey}0.97 & 0.11 \\
        \cmidrule[0.5pt]{1-7}
    \end{tabular}
    \caption{The performance of EgoGaussian and the other baselines on the original EgoGaussian HOI4D data \cite{hoi4d, EgoGaussian}. Ours$^*$ represents the results without metric changes and ours$^\dagger$ represents with the metric changes. Numbers denoted in grey represent the best scoring method across ours$^\dagger$ evaluations. As we can observe, ours$^*$ implementation of EgoGaussian scores similarly to the original. However, we observe that the baselines perform better than EgoGaussian, contrary to the original findings.}
    \label{tab:egogaussian_hoi4d_no_sub_results.tex}
\end{table*}



% \begin{tabular}{|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{|c||}{\textbf{Passive segments}} & \multicolumn{3}{|c|}{\textbf{Active segments}} \\
%         \cline{2-7}
%          & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian (original) \cite{EgoGaussian} & 30.99 & 0.96 & 0.08 & 30.33 & 0.95 & 0.09 \\
%         EgoGaussian (ours$^*$) & 30.52 & 0.96 & 0.09 & 31.12 & 0.96 & 0.09 \\
%         EgoGaussian (ours$^\dagger$) & 30.43 & 0.95 & 0.13 & 30.97 & 0.95 & 0.13 \\
%         \hline
%         Deformable-3DGS (original) \cite{EgoGaussian} & 28.09 & 0.94 & 0.08 & 26.92 & 0.94 & 0.10 \\
%         Deformable-3DGS (ours$^\dagger$) & 34.38 & \textbf{0.97} & \textbf{0.08} & 33.06 & 0.96 & \textbf{0.10} \\
%         \hline
%         4DGS (original) \cite{EgoGaussian} & 28.69 & 0.94 & 0.08 & 27.33 & 0.94 & 0.10 \\
%         4DGS (ours$^\dagger$) & \textbf{36.73} & \textbf{0.97} & 0.09 & \textbf{35.13} & \textbf{0.97} & 0.11 \\
%         \hline
%     \end{tabular}

==> tables/before_bmvc/full_results.tex <==
\begin{table*}[t!]
\begin{adjustwidth}{-2cm}{-2cm}
    \centering
    \begin{tabular}{cccccccc}
        \cmidrule[0.5pt]{1-8}
         &  & \multicolumn{3}{c}{\textbf{Random scenes}} & \multicolumn{3}{c}{\textbf{EgoGaussian scenes}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
        \textbf{Model} & \textbf{View} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-8}
        EgoGaussian & Ego & - & - & - & 27.46 $\pm$ 0.27 & 0.78 $\pm$ 0.002 & 0.31 $\pm$ 0.003 \\
        \cmidrule{1-8}
        \multirow{2}{*}{Def3DGS} & Ego & 30.42 $\pm$ 0.06 & 0.82 $\pm$ 0.004 & 0.27 $\pm$ 0.006 & 29.95 $\pm$ 0.03 & 0.82 $\pm$ 0.000 & 0.25 $\pm$ 0.000 \\
        & Exo & \cellcolor{moderategrey}36.06 $\pm$ 0.04 & \cellcolor{moderategrey}0.97 $\pm$ 0.000 & \cellcolor{moderategrey}0.11 $\pm$ 0.000 & \cellcolor{moderategrey}31.85 $\pm$ 0.11 & \cellcolor{moderategrey}0.93 $\pm$ 0.000 & \cellcolor{moderategrey}0.17 $\pm$ 0.000  \\
        \cmidrule{1-8}
        \multirow{2}{*}{4DGS} & Ego & 29.75 $\pm$ 0.03 & 0.80 $\pm$ 0.001 & 0.32 $\pm$ 0.001 & 29.61 $\pm$ 0.05 & 0.80 $\pm$ 0.001 & 0.30 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}33.23 $\pm$ 0.18 & \cellcolor{moderategrey}0.92 $\pm$ 0.002 & \cellcolor{moderategrey}0.21 $\pm$ 0.003 & \cellcolor{moderategrey}30.47 $\pm$ 0.09 & \cellcolor{moderategrey}0.90 $\pm$ 0.004 & \cellcolor{moderategrey}0.22 $\pm$ 0.006 \\
        \cmidrule{1-8}
        \multirow{2}{*}{RTGS} & Ego & 30.03 $\pm$ 0.02 & 0.81 $\pm$ 0.001 & 0.30 $\pm$ 0.000 & \cellcolor{moderategrey}29.50 $\pm$ 0.01 & 0.81 $\pm$ 0.000 & 0.28 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}32.64 $\pm$ 0.25 & \cellcolor{moderategrey}0.93 $\pm$ 0.006 & \cellcolor{moderategrey}0.17 $\pm$ 0.008 & 29.03 $\pm$ 0.54 & \cellcolor{moderategrey}0.89 $\pm$ 0.008 & \cellcolor{moderategrey}0.22 $\pm$ 0.015 \\
        \cmidrule[0.5pt]{1-8}
    \end{tabular}
\end{adjustwidth}
    \caption{The performance of selected models on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Average performance over 3 training runs is reported alongside the standard deviation. Numbers in grey represent whether the metric was better on the ego or exo view. As we can see, the models perform considerably better on the exo views on average.}
    \label{tab:full_results}
\end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian \cite{EgoGaussian} & Ego & - & - & - & 27.21 & 0.78 & 0.31 \\
%         \hline
%         \multirow{2}{*}{Def3DGS \cite{def3dgs}} & Ego & 30.46 & 0.83 & 0.20 & 29.92 & 0.81 & 0.19 \\
%         & Exo & \textbf{36.04} & \textbf{0.97} & \textbf{0.09} & \textbf{32.00} & \textbf{0.93} & \textbf{0.14}  \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 29.76 & 0.80 & 0.32 & \textbf{29.76} & 0.81 & 0.30 \\
%         & Exo & \textbf{31.86} & \textbf{0.90} & \textbf{0.23} & 28.40 & \textbf{0.88} & \textbf{0.24} \\
%         \hline
%         \multirow{2}{*}{RTGS \cite{rtgs}} & Ego & 30.09 & 0.81 & 0.30 & 29.55 & 0.81 & 0.28 \\
%         & Exo & \textbf{34.93} & \textbf{0.95} & \textbf{0.15} & \textbf{30.44} & \textbf{0.91} & \textbf{0.19} \\
%         \hline
%     \end{tabular}
%     \caption{The performance of selected models on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Bolded numbers represent whether the performance was better on the ego or exo view. As we can see, the models perform considerably better on the exo views.}
%     \label{tab:full_results}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 29.88 & 0.80 & 0.31 & 29.79 & 0.81 & 0.30 \\
%         & Exo & \textbf{33.36} & \textbf{0.92} & \textbf{0.21} & \textbf{30.31} & \textbf{0.90} & \textbf{0.22} \\
%         \hline
%     \end{tabular}
%     \caption{after hypersearch}
%     \label{tab:full_after_hypersearch}
% \end{table*}

==> tables/before_bmvc/hyper_4dgs.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c}
        \textbf{Parameter name} & \textbf{Values} \\
        \hline
        \texttt{grid\_dimensions} & $2$ \\
        \texttt{input\_coordinate\_dim} & $4$ \\
        \texttt{output\_coordinate\_dim} & $16$, $32$ \\
        \texttt{resolution[-1]} & $250$, $150$, $100$, $80$, $75$, $50$, $25$ \\
        \texttt{multires} & [$1$, $2$, $4$], [$1$, $2$] \\
        \texttt{defor\_depth} & $1$, $0$ \\
        \texttt{net\_width} & $128$, $64$ \\
        \texttt{plane\_tv\_weight} & $2.0 \cdot 10^{-4}$, $1.0 \cdot 10^{-4}$ \\
        \texttt{time\_smoothness\_weight} & $1.0 \cdot 10^{-3}$, $1.0 \cdot 10^{-2}$ \\
        \texttt{l1\_time\_planes} & $1.0 \cdot 10^{-4}$ \\
        \texttt{no\_do} & True, False \\
        \texttt{no\_dshs} & True, False \\
        \texttt{no\_ds} & True, False \\
        \texttt{iterations} & $1.4 \cdot 10^{4}$, $1.5 \cdot 10^{4}$, $2.0 \cdot 10^{4}$ \\
        \texttt{batch\_size} & $1$, $2$ \\
        \texttt{coarse\_iterations} & $3.0 \cdot 10^{3}$ \\
        \texttt{densify\_until\_iter} & $1.0 \cdot 10^{4}$, $1.5 \cdot 10^{4}$ \\
        \texttt{opacity\_reset\_interval} & $3.0 \cdot 10^{3}$, $3.0 \cdot 10^{6}$ \\
        \texttt{grid\_lr\_init} & $1.6 \cdot 10^{-3}$ \\
        \texttt{grid\_lr\_final} & $1.6 \cdot 10^{-4}$, $1.6 \cdot 10^{-5}$ \\
        \texttt{opacity\_threshold\_coarse} & $5.0 \cdot 10^{-3}$ \\
        \texttt{opacity\_threshold\_fine\_init} & $5.0 \cdot 10^{-3}$ \\
        \texttt{opacity\_threshold\_fine\_after} & $5.0 \cdot 10^{-3}$ \\
        \texttt{pruning\_interval} & $100$, $8.0 \cdot 10^{3}$ \\
        \texttt{deformation\_lr\_init} & $1.6 \cdot 10^{-4}$ \\
        \texttt{deformation\_lr\_final} & $1.6 \cdot 10^{-5}$, $1.6 \cdot 10^{-6}$ \\
        \texttt{deformation\_lr\_delay\_mult} & $1.0 \cdot 10^{-2}$ \\
    \end{tabular}
    \caption{The hyperparameter search space for 4DGS.}
    \label{tab:hyper_4dgs}
\end{table*}

==> tables/before_bmvc/hyper_def3dgs.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        \textbf{Parameter name} & \textbf{Values} \\
        \hline
        \texttt{iterations} & $1.5 \cdot 10^{4}$, $2.5 \cdot 10^{4}$, $4.0 \cdot 10^{4}$ \\
        \texttt{deform\_depth} & $6$, $8$, $10$ \\
        \texttt{deform\_width} & $128$, $256$, $512$ \\
    \end{tabular}
    \caption{The hyperparameter search space for Deformable-3DGS.}
    \label{tab:hyper_def3dgs}
\end{table}

==> tables/before_bmvc/hyper_rtgs.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        \textbf{Parameter name} & \textbf{Values} \\
        \hline
        \texttt{env\_map\_res} & $0$, $500$ \\
        \texttt{env\_optimize\_until} & $1.0 \cdot 10^{9}$, $5.0 \cdot 10^{3}$ \\
        \texttt{iterations} & $2.0 \cdot 10^{4}$, $3.0 \cdot 10^{4}$ \\
        \texttt{position\_lr\_max\_steps} & $1.5 \cdot 10^{4}$, $3.0 \cdot 10^{4}$ \\
        \texttt{densification\_interval} & $200$, $100$ \\
        \texttt{densify\_until\_iter} & $1.0 \cdot 10^{4}$, $1.5 \cdot 10^{4}$ \\
    \end{tabular}
    \caption{The hyperparameter search space for RTGS.}
    \label{tab:hyper_rtgs}
\end{table}

==> tables/before_bmvc/static_results.tex <==
\begin{table*}[t!]
\begin{adjustwidth}{-2cm}{-2cm}
    \centering
    \begin{tabular}{cccccccc}
        \cmidrule[0.5pt]{1-8}
         &  & \multicolumn{3}{c}{\textbf{Random scenes}} & \multicolumn{3}{c}{\textbf{EgoGaussian scenes}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
        \textbf{Model} & \textbf{View} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-8}
        EgoGaussian & Ego & - & - & - & 27.94 $\pm$ 0.10 & 0.79 $\pm$ 0.001 & 0.30 $\pm$ 0.002 \\
        \cmidrule{1-8}
        \multirow{2}{*}{Def3DGS} & Ego & 31.17 $\pm$ 0.06 & 0.83 $\pm$ 0.004 & 0.27 $\pm$ 0.007 & 30.23 $\pm$ 0.04 & 0.82 $\pm$ 0.000 & 0.25 $\pm$ 0.000 \\
        & Exo & \cellcolor{moderategrey}38.85 $\pm$ 0.01 & \cellcolor{moderategrey}0.97 $\pm$ 0.000 & \cellcolor{moderategrey}0.11 $\pm$ 0.000 & \cellcolor{moderategrey}34.85 $\pm$ 0.08 & \cellcolor{moderategrey}0.96 $\pm$ 0.000 & \cellcolor{moderategrey}0.14 $\pm$ 0.000 \\
        \cmidrule{1-8}
        \multirow{2}{*}{4DGS} & Ego & 30.60 $\pm$ 0.05 & 0.80 $\pm$ 0.001 & 0.31 $\pm$ 0.001 & 29.88 $\pm$ 0.05 & 0.81 $\pm$ 0.001 & 0.30 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}34.56 $\pm$ 0.20 & \cellcolor{moderategrey}0.92 $\pm$ 0.002 & \cellcolor{moderategrey}0.21 $\pm$ 0.003 & \cellcolor{moderategrey}32.45 $\pm$ 0.30 & \cellcolor{moderategrey}0.92 $\pm$ 0.005 & \cellcolor{moderategrey}0.20 $\pm$ 0.007 \\
        \cmidrule{1-8}
        \multirow{2}{*}{RTGS} & Ego & 30.82 $\pm$ 0.02 & 0.82 $\pm$ 0.001 & 0.30 $\pm$ 0.000 & 29.67 $\pm$ 0.01 & 0.82 $\pm$ 0.000 & 0.28 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}33.58 $\pm$ 0.24 & \cellcolor{moderategrey}0.93 $\pm$ 0.006 & \cellcolor{moderategrey}0.17 $\pm$ 0.008 & \cellcolor{moderategrey}30.45 $\pm$ 0.70 & \cellcolor{moderategrey}0.91 $\pm$ 0.010 & \cellcolor{moderategrey}0.20 $\pm$ 0.017 \\
        \cmidrule[0.5pt]{1-8}
    \end{tabular}
\end{adjustwidth}
    \caption{The performance of selected models on static masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Average performance over 3 training runs is reported alongside the standard deviation. Numbers in grey represent whether the performance was better on the ego or exo view. As expected, based on the previous results, the models perform the reconstruction much better for the exo views.}
    \label{tab:static_results}
\end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian \cite{EgoGaussian} & Ego & - & - & - & 27.83 & 0.78 & 0.30 \\
%         \hline
%         \multirow{2}{*}{Def3DGS \cite{def3dgs}} & Ego & 31.23 & 0.83 & 0.20 & 30.18 & 0.82 & 0.18 \\
%         & Exo & \textbf{38.84} & \textbf{0.97} & \textbf{0.08} & \textbf{34.99} & \textbf{0.96} & \textbf{0.11}  \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 30.67 & 0.81 & 0.31 & 30.02 & 0.81 & 0.29 \\
%         & Exo & \textbf{33.04} & \textbf{0.91} & \textbf{0.23} & \textbf{30.80} & \textbf{0.91} & \textbf{0.21} \\
%         \hline
%         \multirow{2}{*}{RTGS \cite{rtgs}} & Ego & 30.74 & 0.82 & 0.30 & 29.70 & 0.82 & 0.28 \\
%         & Exo & \textbf{36.25} & \textbf{0.95} & \textbf{0.15} & \textbf{32.49} & \textbf{0.93} & \textbf{0.17} \\
%         \hline
%     \end{tabular}
%     \caption{The performance of selected models on static masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Bolded numbers represent whether the performance was better on the ego or exo view. As expected, based on the previous results, the models perform the reconstruction much better for the exo views.}
%     \label{tab:static_results}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 30.74 & 0.81 & 0.31 & 30.04 & 0.81 & 0.30 \\
%         & Exo & \textbf{34.66} & \textbf{0.92} & \textbf{0.21} & \textbf{32.31} & \textbf{0.92} & \textbf{0.20} \\
%         \hline
%     \end{tabular}
%     \caption{after hypersearch}
%     \label{tab:static_after_hypersearch}
% \end{table*}



==> tables/egogaussian_hoi4d_no_sub_results.tex <==
\begin{table*}[t!]
    \footnotesize
    \centering
    \begin{tabular}{ccccccc}
        \cmidrule[0.5pt]{1-7}
         & \multicolumn{3}{c}{\textbf{Passive segments}} & \multicolumn{3}{c}{\textbf{Active segments}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        \textbf{Model} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-7}
        EgoGaussian (original) & 30.99 & 0.96 & 0.08 & 30.33 & 0.95 & 0.09 \\
        EgoGaussian (ours$^*$) & 30.52 & 0.96 & 0.09 & 31.12 & 0.96 & 0.09 \\
        EgoGaussian (ours$^\dagger$) & 30.43 & 0.95 & 0.13 & 30.97 & 0.95 & 0.13 \\
        \cmidrule{1-7}
        Def3DGS (original) & 28.09 & 0.94 & 0.08 & 26.92 & 0.94 & 0.10 \\
        Def3DGS (ours$^\dagger$) & 34.38 & \cellcolor{moderategrey}0.97 & \cellcolor{moderategrey}0.08 & 33.06 & 0.96 & \cellcolor{moderategrey}0.10 \\
        \cmidrule{1-7}
        4DGS (original)& 28.69 & 0.94 & 0.08 & 27.33 & 0.94 & 0.10 \\
        4DGS (ours$^\dagger$) & \cellcolor{moderategrey}36.73 & \cellcolor{moderategrey}0.97 & 0.09 & \cellcolor{moderategrey}35.13 & \cellcolor{moderategrey}0.97 & 0.11 \\
        \cmidrule[0.5pt]{1-7}
    \end{tabular}
    \caption{The performance of EgoGaussian and the other baselines on the original EgoGaussian HOI4D data \cite{hoi4d, EgoGaussian}. Ours$^*$ represents the results without metric changes and ours$^\dagger$ represents with the metric changes. Numbers denoted in grey represent the best scoring method across ours$^\dagger$ evaluations. As we can observe, ours$^*$ implementation of EgoGaussian scores similarly to the original. However, we observe that the baselines perform better than EgoGaussian, contrary to the original findings.}
    \label{tab:egogaussian_hoi4d_no_sub_results.tex}
\end{table*}



% \begin{tabular}{|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{|c||}{\textbf{Passive segments}} & \multicolumn{3}{|c|}{\textbf{Active segments}} \\
%         \cline{2-7}
%          & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian (original) \cite{EgoGaussian} & 30.99 & 0.96 & 0.08 & 30.33 & 0.95 & 0.09 \\
%         EgoGaussian (ours$^*$) & 30.52 & 0.96 & 0.09 & 31.12 & 0.96 & 0.09 \\
%         EgoGaussian (ours$^\dagger$) & 30.43 & 0.95 & 0.13 & 30.97 & 0.95 & 0.13 \\
%         \hline
%         Deformable-3DGS (original) \cite{EgoGaussian} & 28.09 & 0.94 & 0.08 & 26.92 & 0.94 & 0.10 \\
%         Deformable-3DGS (ours$^\dagger$) & 34.38 & \textbf{0.97} & \textbf{0.08} & 33.06 & 0.96 & \textbf{0.10} \\
%         \hline
%         4DGS (original) \cite{EgoGaussian} & 28.69 & 0.94 & 0.08 & 27.33 & 0.94 & 0.10 \\
%         4DGS (ours$^\dagger$) & \textbf{36.73} & \textbf{0.97} & 0.09 & \textbf{35.13} & \textbf{0.97} & 0.11 \\
%         \hline
%     \end{tabular}

==> tables/static_results.tex <==
\begin{table*}[t!]
    \footnotesize
    \setlength{\tabcolsep}{3pt}
    \centering
    \begin{tabular}{cccccccc}
        \cmidrule[0.5pt]{1-8}
         &  & \multicolumn{3}{c}{\textbf{Random scenes}} & \multicolumn{3}{c}{\textbf{EgoGaussian scenes}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
        \textbf{Model} & \textbf{View} & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
        \cmidrule{1-8}
        EgoGaussian & Ego & - & - & - & 27.94 $\pm$ 0.10 & 0.79 $\pm$ 0.001 & 0.30 $\pm$ 0.002 \\
        \cmidrule{1-8}
        \multirow{2}{*}{Def3DGS} & Ego & 31.17 $\pm$ 0.06 & 0.83 $\pm$ 0.004 & 0.27 $\pm$ 0.007 & 30.23 $\pm$ 0.04 & 0.82 $\pm$ 0.000 & 0.25 $\pm$ 0.000 \\
        & Exo & \cellcolor{moderategrey}38.85 $\pm$ 0.01 & \cellcolor{moderategrey}0.97 $\pm$ 0.000 & \cellcolor{moderategrey}0.11 $\pm$ 0.000 & \cellcolor{moderategrey}34.85 $\pm$ 0.08 & \cellcolor{moderategrey}0.96 $\pm$ 0.000 & \cellcolor{moderategrey}0.14 $\pm$ 0.000 \\
        \cmidrule{1-8}
        \multirow{2}{*}{4DGS} & Ego & 30.60 $\pm$ 0.05 & 0.80 $\pm$ 0.001 & 0.31 $\pm$ 0.001 & 29.88 $\pm$ 0.05 & 0.81 $\pm$ 0.001 & 0.30 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}34.56 $\pm$ 0.20 & \cellcolor{moderategrey}0.92 $\pm$ 0.002 & \cellcolor{moderategrey}0.21 $\pm$ 0.003 & \cellcolor{moderategrey}32.45 $\pm$ 0.30 & \cellcolor{moderategrey}0.92 $\pm$ 0.005 & \cellcolor{moderategrey}0.20 $\pm$ 0.007 \\
        \cmidrule{1-8}
        \multirow{2}{*}{RTGS} & Ego & 30.82 $\pm$ 0.02 & 0.82 $\pm$ 0.001 & 0.30 $\pm$ 0.000 & 29.67 $\pm$ 0.01 & 0.82 $\pm$ 0.000 & 0.28 $\pm$ 0.002 \\
        & Exo & \cellcolor{moderategrey}33.58 $\pm$ 0.24 & \cellcolor{moderategrey}0.93 $\pm$ 0.006 & \cellcolor{moderategrey}0.17 $\pm$ 0.008 & \cellcolor{moderategrey}30.45 $\pm$ 0.70 & \cellcolor{moderategrey}0.91 $\pm$ 0.010 & \cellcolor{moderategrey}0.20 $\pm$ 0.017 \\
        \cmidrule[0.5pt]{1-8}
    \end{tabular}
    \caption{The performance of selected models on static masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Average performance over 3 training runs is reported alongside the standard deviation. Numbers in grey represent whether the performance was better on the ego or exo view. As expected, based on the previous results, the models perform the reconstruction much better for the exo views.}
    \label{tab:static_results}
\end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         EgoGaussian \cite{EgoGaussian} & Ego & - & - & - & 27.83 & 0.78 & 0.30 \\
%         \hline
%         \multirow{2}{*}{Def3DGS \cite{def3dgs}} & Ego & 31.23 & 0.83 & 0.20 & 30.18 & 0.82 & 0.18 \\
%         & Exo & \textbf{38.84} & \textbf{0.97} & \textbf{0.08} & \textbf{34.99} & \textbf{0.96} & \textbf{0.11}  \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 30.67 & 0.81 & 0.31 & 30.02 & 0.81 & 0.29 \\
%         & Exo & \textbf{33.04} & \textbf{0.91} & \textbf{0.23} & \textbf{30.80} & \textbf{0.91} & \textbf{0.21} \\
%         \hline
%         \multirow{2}{*}{RTGS \cite{rtgs}} & Ego & 30.74 & 0.82 & 0.30 & 29.70 & 0.82 & 0.28 \\
%         & Exo & \textbf{36.25} & \textbf{0.95} & \textbf{0.15} & \textbf{32.49} & \textbf{0.93} & \textbf{0.17} \\
%         \hline
%     \end{tabular}
%     \caption{The performance of selected models on static masks on paired ego and exo views of 8 random scenes and 2 scenes matching EgoGaussian \cite{EgoGaussian} requirements. Bolded numbers represent whether the performance was better on the ego or exo view. As expected, based on the previous results, the models perform the reconstruction much better for the exo views.}
%     \label{tab:static_results}
% \end{table*}

% \begin{table*}[t!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c||c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{View}} & \multicolumn{3}{|c||}{\textbf{Random scenes}} & \multicolumn{3}{|c|}{\textbf{EgoGaussian scenes}} \\
%         \cline{3-8}
%          & & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ & mPSNR $\uparrow$ & mSSIM $\uparrow$ & mLPIPS $\downarrow$ \\
%         \hline
%         \multirow{2}{*}{4DGS \cite{4dgs}} & Ego & 30.74 & 0.81 & 0.31 & 30.04 & 0.81 & 0.30 \\
%         & Exo & \textbf{34.66} & \textbf{0.92} & \textbf{0.21} & \textbf{32.31} & \textbf{0.92} & \textbf{0.20} \\
%         \hline
%     \end{tabular}
%     \caption{after hypersearch}
%     \label{tab:static_after_hypersearch}
% \end{table*}


